kNN-CLIP: Retrieval Enables Training-Free Segmentation on Continually Expanding Large Vocabularies

Continual segmentation has not yet tackled the challenge of improving open-vocabulary segmentation models with training data for accurate segmentation across large, continually expanding vocabularies. We discover that traditional continual training results in severe catastrophic forgetting, failing to outperform a zero-shot segmentation baseline. We introduce a novel training-free strategy, kNN-CLIP, which augments the model with a database of instance embeddings for semantic and panoptic segmentation that achieves zero forgetting. We demonstrate that kNN-CLIP can adapt to continually growing vocabularies without the need for retraining or large memory costs. kNN-CLIP enables open-vocabulary segmentation methods to expand their vocabularies on any domain with a single pass through the data, while only storing compact embeddings. This approach minimizes both compute and memory costs. kNN-CLIP achieves state-of-the-art performance across large-vocabulary semantic and panoptic segmentation datasets. We hope kNN-CLIP represents a significant step forward in enabling more efficient and adaptable continual segmentation, paving the way for advances in real-world large-vocabulary continual segmentation methods.

==> tables/Classification1.tex <==
\begin{table}[t]
  \caption{\textbf{Image Classification Performance.} Retrieval augmentation enhances classification performance of CLIP on Specialized datasets
  }
  \label{tab: Image Classification}
  \centering
  % \resizebox{\textwidth}{!}{%
  \begin{tabular}{@{}c|c|c|c|c@{}}
    \toprule
    Dataset & CLIP-RN50 & SuS-X* & Closed-set KNN-CLIP & Open-source KNN-CLIP\\
    \midrule
    CIFAR10 & 70.31 & 74.95 & 95.80 (+25.49) & 83.15 (+12.84)\\
    CIFAR100 & 35.35 & 44.63 & 87.36 (+52.01) & 68.32 (+32.97)\\
    % ImageNet-A & 23.59 & - & 24.39 (+0.80)\\
    % ImageNet-R & & - &\\
    CUB & 46.69 & 49.12 & 47.00 (+0.31) & 46.85 (+0.16)\\
    Flower & 66.08 & 67.97 & 96.94 (+30.86) & 82.78 (+16.70)\\
    Aircraft & 17.34 & 21.09 & 27.78 (+10.44) & 25.41 (+8.07)\\
    % Cars & 55.63 & 56.05 (+0.42)& -\\
    % EuroSAT & 37.51 & 94.19 (+56.68) & -\\
    % \midrule
  \bottomrule
  \end{tabular}%
  % }
\end{table}

==> tables/InferenceTime.tex <==
\begin{table}[t]
  \caption{\textbf{FPS Comparisons.} All results were obtained using a single A40 GPU with CUDA 11.8 and PyTorch 2.0.0. The average runtime was calculated across the entire validation set and includes post-processing time.
  }
  \label{tab: inference time}
  \centering
  
  \begin{tabular}{@{}c|cc@{}}
    \toprule
    method & ADE20k & COCO\\
    \midrule
    ODISE & 0.41 & 0.39\\
    FC-CLIP & 2.86 & 2.84\\
    \midrule
    RA-FC-CLIP (Brute Force) & 1.31 & 0.83\\
    RA-FC-CLIP(HNSW) & 1.52 & 1.51\\
    % \midrule
  \bottomrule
  \end{tabular}
\end{table}
